Algorithmic Ethics: Formalization and Verification of Autonomous Vehicle Obligations

We develop a formal framework for automatic reasoning about the obligations of autonomous cyber-physical systems, including their social and ethical obligations. Obligations, permissions and prohibitions are distinct from a system's mission, and are a necessary part of specifying advanced, adaptive AI-equipped systems. They need a dedicated deontic logic of obligations to formalize them. Most existing deontic logics lack corresponding algorithms and system models that permit automatic verification. We demonstrate how a particular deontic logic, Dominance Act Utilitarianism (DAU), is a suitable starting point for formalizing the obligations of autonomous systems like self-driving cars. We demonstrate its usefulness by formalizing a subset of Responsibility-Sensitive Safety (RSS) in DAU; RSS is an industrial proposal for how self-driving cars should and should not behave in traffic. We show that certain logical consequences of RSS are undesirable, indicating a need to further refine the proposal. We also demonstrate how obligations can change over time, which is necessary for long-term autonomy. We then demonstrate a model-checking algorithm for DAU formulas on weighted transition systems, and illustrate it by model-checking obligations of a self-driving car controller from the literature.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> analysis-inferring-policies.tex <==
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.4\linewidth]{figs/placeHolder}
%\caption{Standard AV control hierarchy}
%\label{fig:av stack}
%\end{figure}
%
\newcommand{\rssrow}{RSS\ref{rss-row}prohib}
\newcommand{\rssass}{RSS\!\ref{rss-assertive}}

In DAU, obligations are automatically derived from the stit model via Def.~\ref{def:cstit}.
Given an obligation that we \textit{want} the system to have, how should we structure the stit model so that it has that obligation?
This is similar to synthesis-from-specifications, an active research area in programming and in Cyber-Physical Systems.
This section gives an example where it is possible to manually partially infer the stit model structure from the RSS obligations.

Consider again the $\rssrow$ and $\rssass$ statements (Eqs.~\eqref{eq:rss-row prohib 2} and \eqref{eq:rss-assertive}).
 %  - - - - - - - 
 \begin{figure*}[t]
 	\centering
 	\includegraphics[height=2.25in,keepaspectratio]{figs/values}
 	\caption{The optimal action at $m$, $K_1$, necessarily contains history $\tilde{h}$ in which comes a moment $i''$ s.t. $i''/\tilde{h} \models p\land \neg g$. The controller must choose an action, prior to $i''$, that does not contain $\tilde{h}$. Since the controller always chooses optimal actions, the $\Value$ function must favor $K_4$, as shown.}
 	\label{fig:derive policies}
 \end{figure*}
 %
 \begin{proposition}
 	\label{prop:stit model inference}
 	A stit model has both obligations $\rssrow$ and $\rssass$ at $m$ if for every optimal action $K \in \Optimalam$, it holds that $|K|\geq 2$, and there exist a history $\tilde{h} \in K$ and a moment $m'>m$ in $\tilde{h}$ s.t.  $|\Choice{\alpha}{m'}|\geq 2$, $m/\tilde{h} \not\models_{\text{\CTLs}} \always(\neg g_\alpha \implies \neg p_\alpha)$ and $\tilde{h}$ is not in any optimal action at $m'$.
 \end{proposition}
 The conclusion of the Proposition, illustrated in Fig.~\ref{fig:derive policies}, is counter-intuitive: it necessitates the existence of a history $\tilde{h}$ along which one of the formulas, $\always(\neg g_\alpha \implies \neg p_\alpha)$, is \textit{violated}.
 But since the inferred structure places $\tilde{h}$ in a non-optimal action (via $\Value$), this doesn't lead to an \textit{obligation violation}.
\begin{proof}
In this proof we let $[m:n]$ denote the set of integers $\{m,m+1,\ldots, n\}$, and we simplify the notation by writing $g$ and $p$ instead of $g_\alpha$ and $p_\alpha$ for the atomic propositions `$\alpha$ is granted right-of-way' and `$\alpha$ passes through the conflict region', respectively.
%
Starting with $\rssass$, let $A= \neg p \wbuntil g$.
The set of histories $|\dstit{\alpha}{A}|_m = \{h\such m/h\models \dstit{\alpha}{A}\} = \{h \such \Choiceam(h)\subseteq |A|_m\}$ if $H_m\neq|A|_m$, and is empty otherwise. 
Since the case when it is empty is trivial, we focus on the first case in what follows.
Therefore $|\neg\dstit{\alpha}{A}|_m = \{h \such \Choiceam(h) \nsubseteq |A|_m\}$.
%
Now Eq.~\eqref{eq:rss-assertive} says that $\forall K\in \Optimalam/w_\alpha$, $K\subseteq \{h\such \Choiceam(h)\nsubseteq |A|_m\}$, which is equivalent to $K \nsubseteq |A|_m$ (since $\Choiceam(h) = K$ for every $h\in K$).
So for all $K\in \Optimalam/w_\alpha$, $\exists h \in K$ s.t. $m/h \not\models \neg p \wbuntil g$.
From the semantics of $\wbuntil$, this is equivalent to : for all $K\in \Optimalam/w_\alpha$,
\[\exists \tilde{h} \in K \text{ s.t. } \exists i\in [m:m+N]~.~i'/\tilde{h}\models \neg g \forall i' \in [m:i] \text{ but } i''/\tilde{h} \models p \text{ for some } i''\in [m:i] \]

So $i''/\tilde{h}\models p \land \neg g$ and $m/\tilde{h}\models \neg g$, so $m/\tilde{h}\not\models \always(\neg g \implies \neg p)$.
%Moreover $m/\tilde{h}\models \neg g \implies K\cap |\neg g|_m \neq \emptyset \implies K \in \Optimalam/\neg g$.
%Thus a choice of $K$ at $m$ is consistent with both obligations.
If the system evolves along $\tilde{h}$, it risks violating $\rssrow$ at $i''$.
To avoid this, $\tilde{h}$ must not be in any of the optimal actions of $\Optimal{\alpha}{m'}$.
So the $\Value$ function must be designed so that $\Choice{\alpha}{m'}(\tilde{h}) \prec K_3$ for some $K_3 \in \Optimal{\alpha}{m'}$, as shown in Fig.~\ref{fig:derive policies}.
From this we conclude $|\Choice{\alpha}{m'}|\geq 2$ and $|K_1|\geq 2$.
\end{proof}



==> apxMoreDAU.tex <==
\section{More elements of Dominance Act Utilitarianism}
\label{apx:choice}
\textbf{Agent choice}.
The choice mapping $\Choiceam$ in a general deontic stit model obeys
\begin{itemize}
	\item The actions in $\Choiceam$ partition the set $H_m$: $K\cap K' = \emptyset$ for every $K,K'$ and $\cup_{K\in \Choiceam} K = H_m$.
	\item Independence of agents: given any group of agents $\Group \subseteq \Agent$, $\cap_{\alpha\in \Group}\Choiceam  \neq \emptyset$.
	That is, the actions of one agent do not prevent the choice of action available to any other agent at the \textit{same} moment $m$. 
	\item No choice between undivided histories: If two histories are still undivided at $m$ (that is, they share a moment $m'>m$) then they belong to the same action $K$ in $\Choiceam$.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Conditional obligation}.
%%\label{apx:conditional obligation}
%Let $X=|A|_m$ be set of histories satisfying formula $A$ at $m$ in model $\Model$.
%%
%The choice of actions available to $\alpha$ at $m$ under the condition that $X$ holds is defined as $\Choiceam/X \defeq \{K\in \Choiceam \such K\cap X \neq \emptyset\}$. 
%This is the right definition because non-determinism might make it impossible to guarantee $K\subseteq X$ at $m$, but future actions might still ensure the finally realized history $h$ will satisfy $X$.
%Thus in Fig.~\ref{fig:choices} $\Choiceam/B=\{K_1\}$:  even though $K_1$ might lead to, say, $h_1$ where $B$ does not hold, it is a valid choice at $m$, since it could also lead to $h_4$ where $B$ holds.
%%
%Conditional dominance is then naturally defined:
%for two actions $K,K'$ from $\Choiceam$, $K\preceq_X K'$ iff 
%$K\cap S \cap X \leq K'\cap S \cap X$ for all $S \in \State_\alpha^m$.
%%(Compare with Eq.~\ref{eq:action dominance}).
%% 
%The \textit{conditionally optimal actions} are then 
%\begin{equation}
%\label{eq:Optimalam/X}
%\Optimalam/X \defeq \{K \in \Choiceam/X \such \not\exists K' \in \Choiceam/X \textrm{ s.t. } K\prec_X K'\}
%\end{equation}
%%
%Finally, where $A$ and $B$ are formulas, the conditional Ought is defined by
%\begin{equation}
%\label{eq:conditional ought}
%\Model, m/h \models \OstitC{\alpha}{A}{B} \text{ iff } K\subseteq |A|_m^\Model \,\, \forall K \in \Optimalam/|B|_m^\Model.
%\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\textbf{Group actions and obligations.}
%The DAU framework of Section~\ref{sec:dau} can be extended to speak of group actions in a natural way~\cite[Ch. 6]{Horty01DLAgency}. 
%Recall that for a single agent $\alpha$, $\Choiceam$ partitions $H_m$ into disjoint sets of histories.
%Given a set of agents $\Group \subset \Agent$, the set of \emph{group actions available to the group} at moment $m$ is the refinement of this partition by all individual choices. 
%E.g., for 2 agents $\alpha$ and $\beta$, that would be $\Choice{\{\alpha,\beta\}}{m}=\{K_\alpha\cap K_\beta, K_\alpha \in \Choiceam, K_\beta \in \Choice{\beta}{m}\}$.
%And more generally, 
%$\Choice{\Group}{m}=\{\cap_{\alpha \in \Group}K_\alpha, K_\alpha \in \Choiceam, \alpha \in \Group\}$.
%Group obligations are then naturally generalized from the corresponding single agent definitions in Section~\ref{sec:dau}.
%That is, one group action is the intersection of a particular selection of individual actions.
%The set of group actions is the set of all such intersections, taken over the selections of individual actions.

%We now define obligations for a group of agents.
%With $\Group \subseteq \Agent$ a group of agents and $m$ a moment in a utilitarian stit model, set
%$State_\Group^m \defeq \Choice{\Agent \setminus \Group}{m}$.
%Here too, the elements of $State_\Group^m$ are the \textit{background states} against which $\Group$'s actions must be decided.
%
%The dominance relation for groups is then given as follows:
%with $K,K'$ actions in $\Choice{\Group}{m}$, $K\preceq K'$ iff $K\cap S \leq K' \cap S$ for all $S\in State_\Group^m$;
%and $K  \prec K'$ if, in addition, it is not the case that $K' \preceq K$.
%%
%Then 
%\[\Optimal{\Group}{m} \defeq \{K \in \Choice{\Group}{m} . \not\exists K' \in \Choice{\Group}{m}: K \prec K'\}\]

==> apxProofMC.tex <==
\section{Proof of Thm.~\ref{prop:mc is possible}}
\label{apx:proof of mc}

Recall that by executing a stit automaton, a stit model is created (Appendix~\ref{apx: proof of Mt}).

\begin{lemma}
	\label{lemma:Tn'}
	The histories generated by $T_n'$ are exactly the histories of $T$ whose first action is $K_n$, modulo a re-naming of the states.
\end{lemma} 
\begin{proof}
	Recall that $T_n'$ has two components, namely a copy $T_n^{\text{ren}}$ of $T_n$ and a copy of $T$. 
	See Fig.~\ref{fig:algo}.
%		
	$T_n$ is obtained by removing transitions from $T$, thus every history generated by $T_n$ is a valid $T$-history.
%	
	Every history generated by $T_n$ starts with $K_n$ by construction.
	So every history $h$ of $T_n'$ starts with $K_n$, because it starts in $T_n^{\text{ren}}$.
	
	\underline{Case 1: $h$ never leaves $T_n^{\text{ren}}$}.
	$T_n^{\text{ren}}$ is nothing but a renaming of $T_n$ and we've already established that a history of $T_n$ is a history of $T$, so this case is done.
	
	\underline{Case 2: $h$ leaves $T_n^{\text{ren}}$}.
	That is, a transition takes the execution into the $T$ copy. 
	Up to the transition, $h$ is a history of $T$ as established in Case 1. 
	The transition itself, say $(q, K,T.q_I)$, is a valid transition of $T$ (modulo re-naming) since it was created by replacing a $T$ transition of the form $(T.q,T.K, T.q_I)$.
	Once in the $T$ copy, the history of course continues to be a valid history of $T$.
	
\end{proof}


%------------------------------------------------------------------------------------------------------------
\begin{lemma}
	\label{lemma:compute optimalam}
	The set computed at line~\ref{line:optimalam} is indeed $\Optimalar$.
\end{lemma} 
\begin{proof}
	Every history of $T_n'$ starts with $K_n$ so $\vnl = \min\{\Value(h) \such h \in K_n \}$ and $\vnu=\max \{\Value(h) \such h\in K_n\}$.
%	
	By definition of action dominance, $K_n \preceq K_n'$ in $T$ iff $\vnu\leq \vnl'$.
	So $[\vnl,\vnu]$ is un-dominated iff its action $K_n$ is un-dominated and must be optimal.
	
\end{proof}

%------------------------------------------------------------------------------------------------------------
\begin{lemma}
	\label{lemma:false 1}
	If line~\ref{line:false 1} is executed, then $K_n \nsubseteq |A|_{root}$.
\end{lemma} 
\begin{proof}
If $T_n'\not\models \forall A$ this means some execution $\tilde{h}$ of $T_n'$ violates $A$.
By Lemma~\ref{lemma:Tn'} $\tilde{h}$ is also a history of $T$ starting with the optimal action $K_n$, so that $K_n \nsubseteq |A|_{root}$. 
QED.
\end{proof}

%------------------------------------------------------------------------------------------------------------
\begin{lemma}
	\label{lemma:false 2}
	If line~\ref{line:false 2} is executed, then $\Model,root/h\not\models \Ostit{\alpha}{\formula}$
\end{lemma} 
\begin{proof}
	$T \models_{\text{\TenseLogic}} \forall \formula$ iff every history of $T$ satisfies $\formula$ and so $H_{root}=|\formula|_{root}$; in this case, by definition of $dstit$, $root/h \not\models \dstit{\alpha}{\formula}$.
%	
	$T_n'\not\models_{\text{\TenseLogic}} \forall \formula$ iff there exists a history $\tilde{h}$ of $T_n'$ which violates $\formula$.
	Again this is also a history of $T$ which belongs to the optimal $K_n$ so that $K_n \nsubseteq |\formula|_{root}$.

\end{proof}

%------------------------------------------------------------------------------------------------------------
\begin{proof}[Thm.~\ref{prop:mc is possible}]
	We need to establish that the algorithm returns True iff $K\subseteq |A|_{root}$ for every optimal $K$.
	The set of optimal actions is computed at line~\ref{line:optimalam} by Lemma~\ref{lemma:compute optimalam}.
	The for-loop at line~\ref{line:for} visits each optimal action in turn. 
%	
	Line~\ref{line:true} is executed iff none of the `return False' statements preceding it are executed;
	namely, iff $K \subseteq |A|_{root}$ by Lemma~\ref{lemma:false 1} in Case $A$ is \TenseLogic,
	or iff $H\neq |\formula|_{root}$ and $K\subseteq |\formula|_{root}$ in the case of line~\ref{line:dstit pos} by Lemma~\ref{lemma:false 2} 
	(and the case of line~\ref{line:dstit neg} is similarly treated).
	These are the definition of $root/h\models \Ostit{\alpha}{A}$.
	
	For the complexity, the first for-loop takes $2|T|$ operations per iteration to create the automata copies and $2c_\lambda$ to compute $\ell_n$ and $u_n$. Let $\sigma$ be the upper bound on the number of transitions away from any state in $T$. Finding the un-dominated intervals takes at most $\sigma-1$ comparisons to find the largest $\ell_n$ and $\sigma$ to compare each $u_n$ to $\max \ell_n$.
	The second for-loop does at the most two CTL$^*$ model-checking runs per optimal action; each run has complexity $O(|T|\cdot 2^{|\formula|})$ and there are at most $\sigma$ optimal actions.
	The total is then $O(2\sigma(|T|+c_\lambda) + 2\sigma-1 + 2\sigma(|T|2^{|\formula|}))$.

\end{proof}


==> apxProofMDP.tex <==
\section{Proof of Prop.~\ref{prop:find extremal values}}
\label{apx:find extremal values}

\begin{definition}[Stit Markov Decision Process]
	\label{def:stit mdp}
	Let $T = (Q, q_I, \Act, F, \Transrel, L, w,\lambda)$ be a stit automaton.
	A \emph{stit markov decision process} $MDP$ is a tuple $MDP_T = (S, A, P, R)$, where
	\begin{itemize}
      \item $S = Q$ is the finite non-empty set of states. We will use $q, q', \dots$ to refer to states of $MDP_T$,
      \item $A = \Transrel$ is the action space such that there is an action $a$ available to the MDP for each transition in $T$,
      \item $P: S \times A \times S \rightarrow \{0, 1\}$ is the probability $P(q, a, q')$ that the agent goes to $s'$ if it takes action $a$ from state $s$;
      $P(s, a, s') = 1$ if $a = (q, K, q')$ for some $K \in \Act$,
      and $P(s, a, s') = 0$ otherwise,
      \item $R: S \times A \times S \rightarrow \mathbb{R}$ is the reward $R(q, a, q')$ that the agent receives at $q'$ for taking action $a$ from state $q$;
      $R(s, a, s') = w(q, K, q')$ if $a = (q, K, q')$ for some $K \in \Act$, and 
      $R(s, a, s') = -\infty$ otherwise.
    \end{itemize}
\end{definition}

Unlike a stit automaton, the actions available to an MDP are available to it from every state. To prevent the MDP from taking a transition $(q, a, q')$ when $a \not\in \Transrel$, the probability $P(s, a, s')$ of succeeding in taking that transition is 0. This introduces actions to the agent that amounts to waiting in a state. To disincentivize taking wait actions, they are given the weight of $-\infty$.

\begin{proof}
	The policy $\pi^*(q_I)$ found by solving $MDP_{T_n}$ produces the path $\omega^*(q_I)$. From definition \ref{def:stit mdp} the only transitions $(s, a, s')$ that $MDP_{T_n}$ can take without incurring infinite negative reward are those where $(q, K, q') \in \Transrel$ for $T_n$ such that $s=q$ and $s'=q'$. Since the path $\omega^*(q_I)$ maximizes accumulated reward, it will only contain transitions that could be taken in $T_n$. Thus, $\omega^*(q_I)$ corresponds to a single execution of $T_n$; let this execution be $\xi^*$. As $\lambda$ is the same for $MDP_{T_n}$ and $T_n$, then the $\lambda(\xi^*)$ of the execution $\xi^*$ is equal to the value of the optimal path $\omega^*(q_I)$, i.e. $\lambda(\xi^*) = V^*(q_I)$. Further, since $MDP_{T_n}$ can produce any sequence of transitions that $T_n$ can, we know that no execution $\xi$ has a greater $\lambda$-value than $V^*(q_I)$. Therefore, $V^*(q_I)$ is the best possible value of an execution of $T_n$, i.e. $\vnu = V^*(q_I)$.
	
	Similarly, solving $MDP_{T_n^-}$ produces an optimal execution that matches an execution in $T_n^-$. Since $T_n^-$ is a copy of $T_n$ with negated weights, and $\lambda$ is monotonic, the optimal execution of $T_n^-$ is identical to the worst execution of $T_n$. Thus, the $\omega^*(q_I)$ resulting from $MDP_{T_n^-}$ matches the worst execution of $T_n$. Since the weights of transitions in $\omega^*(q_I)$ have merely been negated, we need only negate the discounted sum of weights in $\omega^*(q_I)$ to find the value of the worst execution of $T_n$. Therefore $\vnl = -V^*(q_I)$.
\end{proof}

==> apxProofStitModel.tex <==
\section{Construction of $\Model_T$ and Proof of Thm.~\ref{prop:Mt}}
\label{apx: proof of Mt}


\begin{figure*}[t]
	\centering
	\includegraphics[height=2.3in,keepaspectratio]{figs/mc}
	\caption{Left: a stit model generated by executing the stit automaton $T$ (transition weights not shown). Center and right: Automata $T_n$ and $T_n'$ used in Algorithm~\ref{algo:mc}. $T_1$ only has $K_1$ as first action, and $T_1'$ is obtained by re-naming states of $T_1$ and adding a copy of $T_1$ to it. Executions of $T_1'$ are simply the execution of $T$ that start with $K_1$.}
	\label{fig:algo}
\end{figure*}


We give the formal construction of stit model $\Model_{T,q_0}$ from stit automaton $T$ and state $q_0$, then prove Thm.~\ref{prop:Mt}.
Since $q_0$ is fixed, we drop it from the notation.
We denote by $Post(q,K) = \{q' \such (q,K,q') \in \Transrel\}$ the successors of $q$ under $K$,
and by $Post(q) = \cup_{K \in \Act(q)} Post(q,K)$ all the successors of $q$.
The construction is as follows (see Fig.~\ref{fig:algo}).

\begin{itemize}

\item \textit{Initialization}: set iteration $i=1$, $q = q_0$, $root=0$, $S=\{\langle q_0, 0\rangle \}$, $\Tree = \{0\}$. Integer $i$ tracks the level of the tree.

\item \textit{Expansion}: 
Set $S' = \emptyset$. 
For every couple $\langle q, m\rangle \in S$, %set moment $m=m(q,i-1)$ and 
\begin{enumerate}[Exp1)]
	\item set $\Choiceam = \{K: (q,K,q')\in \Transrel(q) \text{ for some } q'\}$: the agent has a choice of actions at $m$ from the actions that label the transitions out of $q$. \label{expand:1}
	\item For every $K\in \Choiceam$, and every $q' \in Post(q,K)$, let $e=(q,K,q') \in \Transrel$, and add a new moment $m(e,i)$ to $\Tree$ with $m(e,i) > m$, and such that the history ending with the moments $( m,m(e,i))$ belongs to action $K$. 
	Also, add the couple $\langle q',m(e,i)\rangle$ to $S'$. \label{expand:2}
	\item Set the label map $v(m) = L(q)$. \label{expand:3}
\end{enumerate}

\item \textit{Update}: Set $S=S'$.
For the next iteration, set $i=i+1$. 
Goto \textit{Expansion}.

Obviously, this goes on forever if the automaton has cycles and the resulting tree is infinite. 
It remains to define history values.

\item \textit{Valuation}: For every history $h$ constructed in the \textit{Expansion} loop, its value is computed as $\Value(h)=\lambda(w(e_i)_{i\in \Ne})$ where $e_i$'s are the transitions taken while constructing $h$.
\end{itemize}

\begin{proof}[Proof of Prop.~\ref{prop:Mt}]
We first verify that $\Model_T$ is a branching time model (Def.~\ref{def:frame and model}). 
The ordering between moments is irreflexive and transitive by construction. 

Take 3 moments $m_1$, $m_2$ and $m_3$ s.t. $m_1<m_3$ and $m_2<m_3$. 
Moments are only added in Exp\ref{expand:2} so $m_3=m(e,i)$ for some $e=(q,K,q'),i$, and by construction there is a unique moment $m(e',i-1)$ where $e'=(\Tilde{q},K',q)$ at level $i-1$ s.t. $m(e,i)>m(e',i-1)$.
By a simple inductive argument, there is a unique moment $m(e_j,j)$ at level $j$ s.t. $m(e,i)>m(e_j,j)$ for \textit{every} $j<i$. 
Thus the set of moments that are smaller than $m(e,i)$ forms a chain (a linear order) to which must belong both $m_2$ and $m_3$, so either $m_2<m_1$ or $m_1<m_2$.

The tree is rooted at $0$ in the \textit{Initialization} step.

The function $v$ in Exp\ref{expand:3} plays the role of the stit model's label map.

We now show that $\Choiceam$ satisfies the constraints of Appendix~\ref{apx:choice} on choices:
\\
$\bullet$ The actions in $\Choiceam$ partition $H_m$: indeed, take a history starting at $m=m(e,i-1)$. It is expanded in Exp\ref{expand:2} only, by $m(e',i)$, $e'=(q,K',q')$ say, and the expanded history $\langle m,m(e',i)\rangle$ is assigned to only one action, namely $K$. 
Thus the histories $\{\langle m,m(e',i)\rangle \such e' = (q,K',q') \in \Delta\}$ are partitioned among the actions at $m$.
By definition of the automaton transition relation, two different actions must lead to two different states $q'$ and $q''$ so the newly created moments $m(e',i+1)$ and $m(e'',i+1)$ ($e''=(q,K'',q'')$) at the next iteration $i+1$, and which expand these histories, are different.
Therefore, two histories that were in different actions at $m$ will never share a moment after $m$.
Thus the actions at $m$ partition $H_{m}$.
\\
$\bullet$ Independence of agents: this is automatically guaranteed by using an automaton that models the product of all stit automata.
\\
$\bullet$ No choice between undivided histories: as established in the first bullet above, histories that are in different actions at $m$ will never share a moment after $m$.
Therefore, two histories that share a moment at $m'>m$ must be in the same action at $m$.

Finally, $\Choiceam$ is finite for each moment since, as can be seen in Exp\ref{expand:1}, $\Choiceam$ is isomorphic to a subset of $\Delta$ and the latter is finite.
\end{proof}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> proofCMC.tex <==
\section{Proof of Prop.~\ref{prop:cmc is possible}}
\label{apx:proof of cmc}
The difference between checking conditional obligations and unconditional obligations is a matter of finding conditionally optimal actions as opposed to unconditionally optimal actions. Due to this, we refer the reader to Appendix \ref{apx:proof of mc} where relevant.

To prove Thm.~\ref{prop:cmc is possible} we will need the following lemmas:

\begin{lemma}
    \label{lemma:Tnl'}
    The histories generated by all $T_{n,l}'$ are exactly the histories of $T$ whose first action is $K_n$, and satisfy the formula $B$.
\end{lemma}
\begin{proof}
    % Let $T_{n,l}'$ begin as $T_n'$. Consider each transition in the automaton be considered its own action.
    
    % If $\tau = 0$, and $T_{n,l}' \models B$, then $T_{n,l}'$, by lemma \ref{lemma:Tn'}
    $T_{n,l}'$ has two components: a "\textit{fragment}" of $|B|$, followed by a copy of $T$.
    
    Every history generated by \textit{fragment} starts with $K_n$ by construction. Thus every history of $T_{n,l}'$ also starts with $K_n$, since $T_{n,l}'$ starts with a \textit{fragment}.
    
    Every execution of the \textit{fragment} satisfies $B$ in at most $\tau$ steps because every state of \textit{fragment} has only one transition, and transitions to a state that continues to satisfy $B$ by construction. The \textit{fragment} has $\tau$ states; thus $T_{n,l}'$ satisfies $B$, since the horizon of $B$ is limited to $\tau$.
    
    Each transition in \textit{fragment} takes the execution into a state from a copy of $T$. The transition itself is a valid transition of $T$ since it was created by pruning away all but one transition in a copy of $T$. The transition from \textit{fragment} to the final copy of $T$ is a valid transition in the same way. Thus a history generated by $T_{n,l}'$ is a valid history of $T$.
    
    All histories of $T$ whose first action is $K_n$ and satisfy $B$ are generated by the set of all $T_{n, l}'$ since each time a \textit{fragment} grows, a new \textit{fragment} is returned for each transition that could form an automaton that accepts $B$. Thus there is a \textit{fragment} and corresponding $T_{n,l}'$ for each finite history of length $\tau$ that starts with $K_n$ and satisfies $B$.
    \hspace*{\fill}QED.
\end{proof}


%-------------------------------------------------------------------------------
\begin{lemma}
	\label{lemma:compute cond optimalam}
	The set computed at line~\ref{line:condoptimalam} is indeed $\Optimalar/B$.
\end{lemma} 
\begin{proof}
	Every history of each $T_{n,l}'$ starts with $K_n$ so $\vnl = \min\{\Value(h) \such h \in K_n \text{ and } h \models B\}$ and $\vnu=\max \{\Value(h) \such h\in K_n \text{ and } h \models B\}$.
%	
	By definition of action dominance, $K_n \preceq_B K_n'$ in $T$ iff $\vnu\leq \vnl'$.
	So $[\vnl,\vnu]$ is un-dominated iff its action $K_n$ is un-dominated and so is optimal conditioned on $B$.
\end{proof}


%-------------------------------------------------------------------------------

With these lemmas, we can complete the proof for Thm.~\ref{prop:cmc is possible}.
\begin{proof}
	We need to establish that the algorithm returns True iff $K\subseteq |A|_{0}$ for every conditionally optimal $K$.
	The set of conditionally optimal actions is computed at line~\ref{line:condoptimalam} by Lemma~\ref{lemma:compute cond optimalam}.
	By Thm. \ref{prop:mc is possible}, Alg. \ref{algo:mc} returns True iff $K\subseteq |A|_{root}$ for every optimal $K$. Since Alg. \ref{alg:cmc} follows the same procedure for checking conditionally optimal actions, this algorithm must also be correct.
	
	For the complexity, the first for-loop takes $2|T|$ operations per iteration to create the automata copies, the complexity of constructing all $T_{n,l}'$, and $2c_\lambda$ to compute $\ell_{n,l}$ and $u_{n, l}$ for each $T_{n,l}'$.
	
	To compute the complexity of constructing all $T_{n,l}'$, let $\sigma$ be the upper bound on the number of transitions away from any state in $T$. Then, at each step in the recursive calls to Alg. \ref{alg:frag}, there are at most $\sigma$ new automata copies that must be constructed. The complexity of performing \CTLs model-checking on each of these automata is $O(|T|\cdot 2^{|B|})$. In the worst case, every execution of $T$ satisfies $B$. Thus each call to Alg. \ref{alg:frag} executes $\sigma$ calls to itself until $i = \tau$. In totality $l = \sigma^{\tau}$ and Alg. \ref{alg:frag} will have been called $(\sigma^{\tau}-1)/2$ times. This gives each iteration of the first for-loop in Alg. \ref{alg:cmc} a complexity of $O(2|T| + ((\sigma^{\tau}-1)/2)\cdot2|T|\cdot(|T|2^{|B|}) + \sigma^{\tau}\cdot2c_\lambda)$
	
	Finding the un-dominated intervals takes at most $\sigma-1$ comparisons to find the largest $\ell_n$ and at most $\sigma$ to compare each $u_n$ to $\max \ell_n$. The algorithm then proceeds exactly like Alg. \ref{algo:mc} for a total complexity of $O(\sigma(2|T| + ((\sigma^{\tau}-1)/2)\cdot2|T|\cdot(|T|2^{|B|}) + \sigma^{\tau}\cdot2c_\lambda) + 2\sigma-1 + 2\sigma(|T|2^{|\formula|}))$.
\end{proof}


==> propagation-scratch.tex <==
\subsection{Tentative Patterns for Temporal Propagation of Obligations}
%Fundamentally, these are questions about the values we assign to various histories, because these values determine what is optimal at each moment.
%Therefore, a desired propagation pattern yields constraints on the weights of the agent automata from which values are derived, and can be used in designing those automata. 
%Because DAU can be viewed as the logic of utility maximization, logically studying obligation propagation gives a clearer picture of what we commit to, ethically, by making utility maximization the only constraint (or objective) of the agent.
%Specifically, obligations that do not propagate can be considered less important than ones that do; this adds a new, \textit{temporal} ranking of an agent's obligations.
%This is in addition to the ability to rank all obligations that hold at a given moment in time.
%Ultimately, propagation patterns obtainable in DAU are one of the criteria on which to judge its suitability to our purposes, and to determine in what ways it might need to be amended.

Consider first the following tentative propagation patterns, in which $\formula$ and $\psi$ are 
\TenseLogic~formulas:
%obligations (recall Def.~\ref{def:obligation structure}):
\begin{multicols}{2}
	\noindent
	\begin{eqnarray}
		\Ostit{\alpha}{\Next \formula} &\implies & \Next \Ostit{\alpha}{\formula} \label{eq:x false prop ->}
		\\
		\Ostit{\alpha}{\eventually \formula} &\implies& \eventually \Ostit{\alpha}{\formula} \label{eq:ev false prop ->}
%		\\
%		\Ostit{\alpha}{\formula \until \psi} &\implies &  \Ostit{\alpha}{\formula} \until \psi 
	\end{eqnarray}
	\begin{eqnarray}
		\Next\Ostit{\alpha}{ \formula} &\implies &  \Ostit{\alpha}{\Next \formula} \label{eq:x false prop <-}
		\\
		\eventually \Ostit{\alpha}{ \formula} &\implies&  \Ostit{\alpha}{\eventually \formula}  \label{eq:ev false prop <-}
%		\\
%		\Ostit{\alpha}{\formula} \until \psi  &\implies &  \Ostit{\alpha}{\formula \until \psi}
	\end{eqnarray}
\end{multicols}	
\vspace{-.55cm}
\begin{equation}
		\Ostit{\alpha}{\eventually\formula} \land \neg \cstit{\alpha}{\eventually \formula} \land \Next \exists \cstit{\alpha}{\eventually\formula} \implies  \Next \Ostit{\alpha}{\eventually \formula}	\label{eq:big false prop}	
\end{equation}
The first line says that an obligation now to ensure that $\formula$ holds at the next moment is the same as an obligation at the next moment to ensure that $\formula$ holds. 
The second line says the same but with Eventually.
%The third line says that an obligation now to ensure that $\formula$ continuously holds until $\psi$ holds is the same as continuously having an obligation to ensure $\formula$, and that obligation persists only until $\psi$ holds. 
The third says that if the agent now has an obligation to ensure that $\formula$ holds eventually, does not do so now, but it is still possible to do so at the next moment, then at the next moment it still has an obligation to ensure $\formula$ holds eventually. 
At first sight, these patterns seem plausible, at least in some directions of the implications.
However, none are valid in DAU.
\begin{proposition}
	\label{prop:tentative patterns don't hold}
	None of the equations \eqref{eq:x false prop ->}-\eqref{eq:big false prop} is valid in DAU.
\end{proposition}
	\begin{figure}[t]
		\centering
		\begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\linewidth]{figs/cex-next}
            \caption{} \label{fig:cex-next}
          \end{subfigure}%
          \hspace*{\fill}   % maximize separation between the subfigures
          \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\linewidth]{figs/cex-ev}
            \caption{} \label{fig:cex-ev}
          \end{subfigure}%
          \hspace*{\fill}
          \begin{subfigure}{0.3\textwidth}
            \includegraphics[width=\linewidth]{figs/cex-big}
            \caption{} \label{fig:cex-big}
          \end{subfigure}%
		\caption{Counter-examples to tentative obligation propagation patterns. (a) Next, Eqs.~\eqref{eq:x false prop ->},\eqref{eq:x false prop <-};  (b) Eventually, Eqs.~\eqref{eq:ev false prop ->},\eqref{eq:ev false prop <-}; (c) Big, Eq.~\eqref{eq:big false prop}}
		\label{fig:cex}
	\end{figure}
	
\begin{proof}
See Fig.~\ref{fig:cex} for counter-examples to each pattern.

In Fig. \ref{fig:cex-next}, $m_1/h \models \Ostit{\alpha}{\Next \phi}$, but since it is not the case that $m_3/h \models \Ostit{\alpha}{\phi}$, Eq. \eqref{eq:x false prop ->} is false. Also, though it is the case that $m_1/h \models \Next \Ostit{\alpha}{\Next \psi}$ (since $m_3/h \models \Ostit{\alpha}{\psi}$), $m_1/h \not\models \Ostit{\alpha}{\Next \psi}$, so Eq. \eqref{eq:x false prop <-} is false.

In Fig. \ref{fig:cex-ev}, for $\forall h \in \Optimal{\alpha}{m_1}$, $\exists m_h \text{ s.t. } m_h/h \models \phi$. This ensures $m_1/h \models \Ostit{\alpha}{\eventually \phi}$. In this example, $m_h \not= m_{h'} \forall h \not= h'$. These moments are shown as points along histories in the figure. Thus, at $m'$, the only history in $\Optimal{\alpha}{m'}$ ($h_3$) does not guarantee $\phi$, so $m'/h \not\models \Ostit{\alpha}{\phi}$, $m_1/h \not\models \eventually \Ostit{\alpha}{\phi}$, and Eq. \eqref{eq:ev false prop ->} is proven false. Alternatively, if $\value{h_2}>\value{h_3}$ and $h_3$ never satisfies $\phi$, then $m_1/h \models \eventually \Ostit{\alpha}{\phi}$, but $m_1/h \not\models \Ostit{\alpha}{\eventually \phi}$, so Eq. \eqref{eq:ev false prop <-} is false.

In Fig. \ref{fig:cex-big}, it is the case that $m_1/h \models \Ostit{\alpha}{\eventually \phi}$, and that $\Next \exists \cstit{\alpha}{\eventually \phi}$. If $K_2$ will be taken, then $\eventually \phi$ is not guaranteed, and $m_2/h \not\models \Ostit{\alpha}{\eventually \phi}$, so Eq. \eqref{eq:big false prop} must also be false.
\end{proof}
In disproving the preceding patterns with Next, we have leveraged the fact that the history along which the formula is evaluated is not necessarily optimal - that is, the agent could take a non-optimal action. 
%In other words, just because an obligation holds now, we should not expect that it will induce an obligation at the next moment; a non-optimal action creates a new situation that is unrelated to the optimal futures from the previous moment. 
And in disproving the patterns with Eventually, we leveraged the fact that obligations that hold at a future moment $m'>m$ depend on the relative values of histories that branch \textit{at that moment}, not of histories that branch at the current moment $m$. 
Thus, when trying to establish propagation patterns, there is a need to factor in the agent's actions, and the values of histories in those actions, whether they are optimal or not.
The next sub-section does that.



\subsection{DAU Propagation Patterns}
\label{sec:dau propagation patterns}

We present three DAU propagation patterns and their conditions of validity.
We will need to express, in the logic, that $\alpha$ took an optimal action. 
So we define the distinguished atomic proposition $\atakopt$ for this purpose:
\[m/h\models \atakopt \text{  iff  } \Choiceam(h) \in \Optimalam\]

The first two patterns are valid by virtue of the fact that they assume $\alpha$ acts optimally. 
\begin{eqnarray}
\label{eq:pattern1}
\Ostit{\alpha}{\Next \formula} \land \atakopt &\implies& \Next \Ostit{\alpha}{\formula}
\\
\Ostit{\alpha}{\eventually \formula} \land  \atakopt \land \forall \neg \formula &\implies& \Next \Ostit{\alpha}{\eventually\formula} \label{eq:simple prop ev}
\end{eqnarray}
Contrast \eqref{eq:simple prop ev} with \eqref{eq:big false prop}.
Note that $\forall \neg \formula$ is necessary for~\eqref{eq:simple prop ev}; the implication fails without it.

We are now ready to present a more general pattern of obligation propagation, which is satisfied only by models whose history values obey certain constraints.
Recall that $m^+(h)$ is the moment that follows $m$ in history $h$.

\begin{proposition}
	\label{prop:ob prop general}
	With $\formula,\psi$ \TenseLogic~formulas, let $\Model$ be a stit model which satisfies the following constraint at every moment $m$:
	for all actions $K \in \Choiceam$ s.t. $K\subseteq |\neg \formula|_m$ and which contain a history $h$ s.t. 
	$m^+(h) \models \exists \cstit{\alpha}{\psi}$,
	it holds that all optimal actions in $\Optimal{\alpha}{m^+(h)}$ guarantee $\psi$.
	(History $h$ is equivalently characterized by $\exists K' \in \Choice{\alpha}{m^+(h)}~.~K' \subset |\psi|_{m^+(h)}$).
	Then \textit{in such a model}, the following is satisfied at every index $m/h$.
	\begin{equation}
	\label{eq:ob prop general}
	\Ostit{\alpha}{\formula \lor \Next \psi} \land \cstit{\alpha}{\neg \formula } \land \Next \exists \cstit{\alpha}{\psi} \implies \Next \Ostit{\alpha}{\psi}
	\end{equation}	
\end{proposition}
The antecedent $\Next \exists \cstit{\alpha}{\psi}$ ensures that at the next moment, $\alpha$ \textit{can} see to it that $\psi$ holds. 
This is needed in general since impossible obligations are not allowed in DAU.
\begin{proof}
	Let $m/h$ be an index in $\Model$ at which the DAU formula \eqref{eq:ob prop general} is evaluated.
	Let $K_h$ be the action to which $h$ belongs,
	and for brevity, write $m' = m^+(h)$.
	
	\underline{Case 1: $h \in \cup_{K\in \Optimalam} K$.}
	Then $K_h\subseteq |\formula \lor \Next \psi|_m = |\formula|_m \cup |\Next \psi|_m$.
	By hypothesis, $K_h \subseteq |\neg \formula|_m$ also so 
	$K_h \subseteq |\Next \psi |_m \setminus |\neg \formula|_m$.	
	By construction, $\Optimal{\alpha}{m'}\subseteq H_{m'} \subseteq K_h$ so for every $K^* \in \Optimal{\alpha}{m'}$ and every $h'\in K^*$, $m'/h'\models \psi$, 
	which is the definition of $m/h \models \Next \Ostit{\alpha}{\psi}$.
	%Note that in this case, the antecedent $\Next \exists \cstit{\alpha}{\psi}$ is redundant. 
	
	\underline{Case 2: $h \notin \cup_{K\in \Optimalam} K$.}
	Fig.??? \todo{@Houssam: what figure is this? I don't remember discussing it. Do you have a rough idea of how it should look? Let me know and I can draw it up.} shows the need for the constraint on the models in this proposition. 
	The figure shows a tree where the antecedent of \eqref{eq:ob prop general} is true, but the conclusion fails. 
	The reason it fails is that the action at $m'$ which guarantees $\psi$ is not optimal. 
	The constraint on the model imposes optimality.
	Formally: from the formula antecedent, we have that $K_h \subseteq |\neg \formula|_m$ and that $m'/h \models \exists \cstit{\alpha}{\psi}$. 
	Therefore the model constraint yields that all optimal actions at $m'$ guarantee $\psi$, which is the definition of $m/h\models \Next \Ostit{\alpha}{\psi}$.	
\end{proof}

The proposition's proof also establishes the following simpler pattern.
\begin{corollary}
	\label{cor:ob prop}
	The following is valid (i.e., satisfied in all models) in DAU:
	\[\Ostit{\alpha}{\formula \lor \Next \psi} \land \cstit{\alpha}{\neg \formula } \land \atakopt \implies \Next \Ostit{\alpha}{\psi}\]
\end{corollary}

==> rss-assertive.tex <==


